When Every Simulation Counts: Value-Based Reinforcement Learning for Accelerated Photonics Inverse Design

Photonic-crystal surface-emitting lasers (PCSELs) can combine high-power operation with narrow-divergence surface emission, but optimizing coupled parameters requires costly full-wave simulations. Deep Q-network (DQN) optimization can reuse simulated transitions to guide edits, yet which value-learning mechanisms remain reliable under tight simulation budgets is unknown. We address this gap by comparing baseline DQN and six value-based variants for a seven-variable PCSEL design under a shared objective, simulator, 83-call budget, and four matched initializations. Beyond endpoints, we analyze sample efficiency, policy behavior, and physical response to separate learning gains from favorable starts or exploratory jumps. Dueling DQN is the only variant to improve all four seeds. Relative to the first evaluated designs, its selected structures increase the mean quality factor () from to (), reduce wavelength error by 64%, and increase upward power by 47%; compared with baseline DQN, they achieve a higher mean under the same budget. Other variants yield no consistent improvement; Double DQN reproduces baseline trajectories, while Rainbow-lite shows high upside but strong seed dependence. These results identify Dueling DQN as the most reliable configuration tested for simulation-budget-limited PCSEL inverse design and provide a reproducible framework for attributing algorithmic gains in scientific optimization. The source code is publicly available at https://github.com/Longying-Wen/PCSEL-RL.

==> tables_current_best_physical_metrics.tex <==
\begin{tabular}{rrrrrrrr}
\toprule
Seed & Score & Call & $Q$ ($10^6$) & $\lambda$ (nm) & $P$ & $A_\mathrm{eff}$ ($10^{-13}$) & $\theta$ (deg) \\
\midrule
0 & 88.701 & 47 & 1.378 & 1310.514 & 0.104 & 0.811 & 0.841 \\
1 & 97.283 & 64 & 4.533 & 1310.132 & 0.124 & 0.805 & 0.841 \\
2 & 94.371 & 42 & 4.596 & 1309.750 & 0.066 & 0.879 & 0.841 \\
3 & 94.045 & 78 & 12.015 & 1310.132 & 0.062 & 0.830 & 0.841 \\
\bottomrule
\end{tabular}


==> tables_current_compact_comparison.tex <==
\begin{tabular}{lrrrrrrrrrr}
\toprule
& \multicolumn{3}{c}{Endpoint} & \multicolumn{2}{c}{Efficiency} & \multicolumn{2}{c}{Robustness} & \multicolumn{3}{c}{Physical response} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}\cmidrule(lr){9-11}
Model & Mean best & Min. & Std. & AUC & Top-5 & $\geq$90 seeds & Policy $\geq$83 & $Q$ ($10^6$) & $|\Delta\lambda|$ & $P$ \\
\midrule
DQN & 87.51 & 84.65 & 3.59 & 84.35 & 85.77 & 1/4 & 3.00 & 2.19 & 0.86 & 0.078 \\
\textbf{Dueling} & \textbf{93.60} & \textbf{88.70} & 3.58 & \textbf{89.22} & \textbf{93.12} & \textbf{3/4} & 7.25 & \textbf{5.63} & \textbf{0.26} & \textbf{0.089} \\
Distributional & 85.92 & 84.04 & \textbf{1.74} & 83.76 & 84.92 & 0/4 & 5.00 & 1.32 & 0.95 & 0.083 \\
PER & 87.49 & 84.72 & 4.30 & 84.08 & 85.25 & 1/4 & 1.00 & 2.61 & 0.93 & \textbf{0.089} \\
Noisy & 87.70 & 85.20 & 4.34 & 85.52 & 85.16 & 1/4 & 5.50 & 1.83 & 0.98 & 0.086 \\
Double & 87.51 & 84.65 & 3.59 & 84.35 & 85.77 & 1/4 & 3.00 & 2.19 & 0.86 & 0.078 \\
Rainbow-lite & 88.01 & 78.62 & 9.29 & 84.78 & 87.22 & 2/4 & \textbf{15.75} & 2.40 & 0.35 & 0.075 \\
\bottomrule
\end{tabular}


==> tables_current_dqn_variant_comparison.tex <==
\begin{tabular}{rrrrrrrrrrrrrr}
\toprule
Seed & DQN best & Dueling best & Dueling gain & Dist. best & Dist. gain & PER best & PER gain & Noisy best & Noisy gain & Double best & Double gain & Rainbow best & Rainbow gain \\
\midrule
0 & 85.20@20 & 88.70@47 & +3.50 & 85.20@20 & +0.00 & 85.20@20 & +0.00 & 85.20@20 & +0.00 & 85.20@20 & +0.00 & 96.54@60 & +11.34 \\
1 & 87.66@67 & 97.28@64 & +9.63 & 88.13@67 & +0.47 & 86.18@51 & -1.48 & 86.14@40 & -1.52 & 87.66@67 & +0.00 & 95.43@35 & +7.78 \\
2 & 92.51@79 & 94.37@42 & +1.86 & 86.33@58 & -6.18 & 84.72@56 & -7.80 & 85.31@54 & -7.21 & 92.51@79 & +0.00 & 78.62@64 & -13.90 \\
3 & 84.65@70 & 94.04@78 & +9.39 & 84.04@54 & -0.61 & 93.88@78 & +9.22 & 94.18@66 & +9.53 & 84.65@70 & +0.00 & 81.46@24 & -3.20 \\
\midrule
Mean & 87.51 & 93.60 & +6.09 & 85.92 & -1.58 & 87.49 & -0.01 & 87.70 & +0.20 & 87.51 & +0.00 & 88.01 & +0.51 \\
\bottomrule
\end{tabular}


==> tables_current_environment_controls.tex <==
\begin{tabular}{lrrrr}
\toprule
Control & Initial value & Admissible range & Increment & Actions ($+/-$) \\
\midrule
$w$ (masked) & 2075 nm & 1000--3000 nm & 25 nm & 0/1 \\
$t$ & 455.0 nm & 350--550 nm & 2.5 nm & 2/3 \\
$t_1$ & 45.0 nm & 0--200 nm & 2.5 nm & 4/5 \\
$t_3$ & 287.5 nm & 215--415 nm & 2.5 nm & 6/7 \\
$n_1=n_4$ & 3.2035 & 3.0535--3.3535 & 0.005 & 8/9 \\
$n_3$ & 3.4250 & 3.265--3.565 & 0.005 & 10/11 \\
$\ell$ & 0.5796875 & 0.22--0.82 & 0.005 & 12/13 \\
$a$ & 400.0 nm & 300--500 nm & 2.5 nm & 14/15 \\
\bottomrule
\end{tabular}


==> tables_current_extended_comparison.tex <==
{\small\textit{(a) Comprehensive benchmark.}}\par\smallskip
\resizebox{\textwidth}{!}{%
\begin{tabular}{lrrrrrrrrrrrrrr}
\toprule
& \multicolumn{3}{c}{Endpoint quality} & \multicolumn{2}{c}{Sample efficiency} & \multicolumn{3}{c}{Candidate discovery} & Policy & \multicolumn{4}{c}{Physical response} & Overall \\
\cmidrule(lr){2-4}\cmidrule(lr){5-6}\cmidrule(lr){7-9}\cmidrule(lr){10-10}\cmidrule(lr){11-14}\cmidrule(lr){15-15}
Model & Mean best & Min best & Std. & AUC & First $\geq$83 & $\geq$90 seeds & Top-5 & $\geq$90 calls & $\geq$83 calls & $Q$ ($10^6$) & $|\Delta\lambda|$ & $P$ & $A_\mathrm{eff}$ ($10^{-13}$) & Avg. rank \\
\midrule
DQN & 87.51 & 84.65 & 3.59 & 84.35 & 37.2 & 1/4 & 85.77 & 0.50 & 3.00 & 2.19 & 0.86 & 0.078 & 0.80 & 4.54 \\
\textbf{Dueling} & \textbf{93.60} & \textbf{88.70} & 3.58 & \textbf{89.22} & 29.8 & \textbf{3/4} & \textbf{93.12} & \textbf{12.50} & 7.25 & \textbf{5.63} & \textbf{0.26} & \textbf{0.089} & \textbf{0.83} & \textbf{1.23} \\
Dist. & 85.92 & 84.04 & \textbf{1.74} & 83.76 & 37.8 & 0/4 & 84.92 & 0.00 & 5.00 & 1.32 & 0.95 & 0.083 & 0.81 & 5.54 \\
PER & 87.49 & 84.72 & 4.30 & 84.08 & 40.5 & 1/4 & 85.25 & 0.50 & 1.00 & 2.61 & 0.93 & 0.089 & 0.81 & 4.65 \\
Noisy & 87.70 & 85.20 & 4.34 & 85.52 & 32.5 & 1/4 & 85.16 & 0.25 & 5.50 & 1.83 & 0.98 & 0.086 & 0.80 & 4.35 \\
Double & 87.51 & 84.65 & 3.59 & 84.35 & 37.2 & 1/4 & 85.77 & 0.50 & 3.00 & 2.19 & 0.86 & 0.078 & 0.80 & 4.54 \\
Rainbow & 88.01 & 78.62 & 9.29 & 84.78 & \textbf{21.5} & 2/4 & 87.22 & 11.00 & \textbf{15.75} & 2.40 & 0.35 & 0.075 & 0.83 & 3.15 \\
\bottomrule
\end{tabular}

}
\par\medskip
{\small\textit{(b) Complementary process statistics.}}\par\smallskip
\resizebox{0.68\textwidth}{!}{%
\begin{tabular}{lrrrr}
\toprule
Model & Post-init. mean & Calls 64--83 mean & $\geq$83 calls & Non-exploratory mean \\
\midrule
DQN & 74.88 & 76.79 & 8.75 & 73.55 \\
Dueling & 77.40 & 79.69 & 21.00 & 75.34 \\
Dist. & 74.66 & 76.34 & 9.00 & 73.84 \\
PER & 74.26 & 75.50 & 6.50 & 73.44 \\
Noisy & 74.54 & 74.98 & 5.50 & 74.54 \\
Double & 74.88 & 76.79 & 8.75 & 73.55 \\
Rainbow & 77.67 & 80.40 & 15.75 & 77.67 \\
\bottomrule
\end{tabular}

}


==> tables_current_shared_training_settings.tex <==
\begin{tabular}{@{}p{0.19\textwidth}p{0.75\textwidth}@{}}
\toprule
Setting & Shared implementation \\
\midrule
State scaling & Divide $[\Delta w,\Delta t,\Delta t_1,\Delta t_3,\Delta n_1,\Delta n_3,\Delta\ell,\Delta a]$ by $[1500,150,150,150,0.225,0.225,0.45,150]$ and clip componentwise to $[-1,1]$; dimensional entries are in nm. \\
Network and actions & ReLU MLP $8$--$80$--$120$--$80$ with 16 compatibility outputs; width actions 0 and 1 are masked, leaving 14 selectable edits. \\
Optimization & Adam, learning rate $10^{-4}$; $\gamma=0.98$; batch size 16; replay capacity 3500. Scalar agents use Smooth-L1 loss and C51 agents use projected categorical cross-entropy. \\
Gradient and target updates & Each gradient element is clipped to $[-1,1]$; one gradient update follows each learned call, and the target network is copied every 50 action selections. \\
Simulation budget & 83 FDTD calls per run. Calls 1--20 are forced-uniform-random transitions stored without learning; learning starts at call 21. \\
Epsilon schedule & $\epsilon_k=0.10+0.55\exp(-k/500)$, where $k$ includes the 20 initialization calls; Noisy DQN and Rainbow-lite set post-initialization epsilon to zero. \\
Local-search protocol & Calls 21--83 form 21 three-edit incumbent-reset windows. Replay remains one-step, $r_k=S(\mathbf{s}_{k+1})$, and the sequence-bonus weight is zero. \\
Reproducibility & Seeds 0--3 set Python, NumPy, and PyTorch generators; all 28 selected configurations record CPU execution. \\
\bottomrule
\end{tabular}


==> tables_current_variant_implementation.tex <==
\begin{tabular}{@{}p{0.13\textwidth}p{0.43\textwidth}p{0.16\textwidth}p{0.17\textwidth}@{}}
\toprule
Agent & Output or target modification & Replay & Exploration \\
\midrule
DQN & Scalar 16-action head; standard target-network maximum. & Uniform & Epsilon-greedy \\
Dueling DQN & Scalar value and 16-action advantage heads; advantages are mean-centered over all 16 compatibility outputs before masking. & Uniform & Epsilon-greedy \\
Distributional DQN & $16\times51$ categorical outputs and C51 projection on $[0,5000]$. & Uniform & Epsilon-greedy \\
PER-DQN & Baseline scalar network and target. & Proportional PER & Epsilon-greedy \\
Noisy DQN & Factorized-Gaussian NoisyLinear second and third hidden layers and output head. & Uniform & Parameter noise \\
Double DQN & Online-network action selection and target-network evaluation. & Uniform & Epsilon-greedy \\
Rainbow-lite DQN & Noisy dueling categorical head with a Double target; combines Dueling, C51, PER, NoisyLinear, and Double DQN without multi-step returns. & Proportional PER & Parameter noise \\
\bottomrule
\end{tabular}

